Subgraph Retrieval Enhanced Model for Multi-hop Knowledge Base Question Answering

Recent works on knowledge base question answering (KBQA) retrieve subgraphs for easier reasoning. A desired subgraph is crucial as a small one may exclude the answer but a large one might introduce more noises. However, the existing retrieval is either heuristic or interwoven with the reasoning, causing reasoning on the partial subgraphs, which increases the reasoning bias when the intermediate supervision is missing. This paper proposes a trainable subgraph retriever (SR) decoupled from the subsequent reasoning process, which enables a plug-and-play framework to enhance any subgraph-oriented KBQA model. Extensive experiments demonstrate SR achieves significantly better retrieval and QA performance than existing retrieval methods. Via weakly supervised pre-training as well as the end-to-end fine-tuning, SRl achieves new state-of-the-art performance when combined with NSM, a subgraph-oriented reasoner, for embedding-based KBQA methods.

==> backup/introduction.tex <==


\section{Introduction}
\label{sec:introduction}

%Knowledge bases (KBs) such as Freebase, Wikidata, DBPedia, Yago, NELL can be viewed as a collection of real-world facts, where each fact is specified as a triplet (head entity, relation, tail entity). 
Knowledge Base Question Answering (KBQA) aims to seek the answers of the factoid questions from the structured KBs such as Freebase, Wikidata, and DBPedia. KBQA has attracted a lot of attention~\cite{bao-etal-2016-constraint,lan-jiang-2020-query,sun2020sparqa,kapanipathi2021leveraging}, as the logically organized entities and their relations are beneficial for the answer reasoning process. 

\begin{figure}[t]
	\centering
	\subfigure[WebQSP]{\label{subfig:grapft-net}
		\includegraphics[width=0.23\textwidth]{Figures/ppr_on_webqsp}
	}
	\hspace{-0.1in}
	\subfigure[CWQ]{\label{subfig:grapft-net}
		\includegraphics[width=0.23\textwidth]{Figures/ppr_on_cwq}
	}
	\caption{\label{fig:graphsize} The impact of various subgraps on QA performance on (a) WebQSP (b) CWQ. }
\end{figure}

Two mainstream approaches that are commonly known as semantic parsing-based (SP-based) methods and information retrieval-based (IR-based) methods have been proposed to solve KBQA. The former approaches translate the textural question into a logic form that can be directly executed against the KB to obtain the answer~\cite{chen2019bidirectional,miller2016key,qiu2020stepwise,saxena-etal-2020-improving,xu-etal-2019-enhancing,zhou-etal-2018-interpretable}. However, this SP-based approaches are less fault-tolerant, as they rely heavily on the accuracy of the parsed executable logic form. Instead of parsing the question, the IR-based approaches first retrieve a question-relevant subgraph from the whole KB and then infer the answers from the subgraph based on its relevance with the question~\cite{He_2021,sun-etal-2018-open,SunACL2019}. The retriever is crucial as it is infeasible to examine the entire space of the subgraph and meanwhile the retrieval accuracy bounds the performance of the next answer reasoning process.


Existing IR-based approaches retrieve the multi-hop neighbors and relations starting from the topic entities to compose the subgraph\footnote{Entities mentioned in a question are referred to as the topic entities.}~\cite{He_2021,sun-etal-2018-open,SunACL2019}. However, this heuristic retrieving methods are far from optimal, since the resultant subgraph is either much larger than necessary to include noises or is inadequate to cover the answer. Figure~\ref{fig:graphsize} presents the Hits@1 performance of two well-known IR-based methods, GRAFT-Net~\cite{sun-etal-2018-open} and NSM~\cite{He_2021}, over different sizes of the heuristically retrieved subgraphs. Specifically, they perform the Personalized PageRank (PPR)~\cite{haveliwala2003topic} to expand the relevant relations and entities to the question. Each entity is attached with a PPR score that can be used to filter the entities to control the size of the subgraph. From the results, we can see that with the increase of the subgraph size, the coverage rate of the answers rises but the reasoning accuracy of the answers falls, which demonstrates the crucial role of the subgraph quality. Besides, the retrieval time increases exponentially with the neighbor hops, which is infeasible in practice.  

Some researchers are aware of the problem and propose a retriever learning strategy instead of the above ad hoc retrieving strategy. For example, PullNet~\cite{SunACL2019} is such an iterative method to learn the retriever. At each iteration, a LSTM-based retriever filters a new fact based its relevance to the question, and then a GNN-based reasoner determines to add the entity of a new fact into the subgraph based on its classifying result on the subgraph. The retrieving and the reasoning are intertwined at each iteration, which is unbeneficial for the reasoner to make the intermediate decisions as the intermediate supervision signals are usually missing. Making decisions on the entire evidences, i.e., the whole subgraph instead of the partially retrieved subgraph, could be easier for the reasoner.


To address the above problem, this paper frames the KBQA task as \textbf{a two separated steps, i.e., ``Subgraph-Retrieving'' and ``Answer-Reasoning''}, where an efficient-oriented retriever firstly obtains a relevant subgraph and then a delicately-devised reasoner deduces the answer from the subgraph. The framework can be explained by the dual process theory in cognitive science~\cite{evans2003two,evans2008dual} which suggests that given an request, the human brains first retrieve relevant information via an implicit, unconscious and intuitive process called System 1, based on which another explicit, conscious and controllable reasoning process, System 2, is then conducted~\cite{ding2019cognitive}. The simple system1 and complex system2 enable fast and slow thinking of the brain~\cite{daniel2017thinking}, which can be corresponded to the retriever and the reasoner respectively.
The same idea is also widely studied in open domain document-based question answering
%where the retriever is responsible for quickly seeking relevant documents as evidences to the question and the reasoner is to carefully infer the answers from the evidences
~\cite{guu2020retrieval,lee2019latent,sachan2021end}. However, retrieving a high-quality subgraph from the KB is different from document retrieval. Thus it deserves careful investigation. 


To enable this fast retrieving and slow reasoning, 
an efficient dual-encoder is devised as the retriever to process the question and each relation path\footnote{A relation path, being composed by a sequence of relations, can be generalized across entities.} that can induce a subgraph. 
The framework can be adapted to any IR-based KBQA model such as GRAFT-Net~\cite{sun-etal-2018-open} or NSM~\cite{He_2021} by solely specify the reasoner in the framework as the existing model.
%The retriever learns $K$ relation paths, induces a subgraph by each path and fuses all the $K$ subgraphs into a single subgraph. Then the reasoner takes as input the fused subgraph and the question to predict the answer.

To teach the retriever by the direct supervised signals from the answers, we propose an end-to-end training strategy for optimizing the retriever and the reasoner. 
%Specifically, given a subgraph as a hidden variable, the retriever can be viewed as a prior distribution to infer the underlying subgraph, while the reasoner computes the likelihood distribution of the answer conditioned on the retrieved subgraph.
Specifically, at each training iteration, we first generate $K$ paths by the retriever, and then update the reasoner's parameters via predicting the answers on the fusion of $K$ subgraphs induced by those paths. Then an EM algorithm is adopted to update the retriever by maximizing the posterior probabilities of the sampled paths. Essentially, the supervision from the answer is enabled by injecting the likelihood of the answer conditioned on a subgraph as the feedback into the prior distribution of the subgraph.  

The end-to-end training is still challenging since we need to learn what to retrieve and which is the correct answer on a subgraph. To improve the model robustness, we  explore two additional pre-training strategies. The first is the weak-supervised pretraining which derives the shortest paths from the topic entities in the question and the answer as the supervision signals. The second one is the unsupervised pretraining which does not reply on the QA pairs, but retrieves the sentences that can explain the relations in a path successively as the augmented dataset.

A series of experiments on WebQSP~\cite{yih-etal-2016-value} and CWQ~\cite{talmor-berant-2018-web} show that: (1) the two-step framework performs much better than the current state-of-the-art IR-based KBQA models (+XX-XX\% Hits@1); (2) the proposed retriever, combined with any IR-based reasoner, achieves significant gains (+XX-XX\% Hits@1) over the same reasoner but with other retrieving strategies;
(3) the end-to-end training method can enhance the performance of both the retriever (+XX-XX\% Hits@1) and the reasoner (+XX-XX\% Hits@1); (4) the pre-training strategies can crucially improve the retriever (+XX-XX\% Hits@1) and also boost the reasoner (+XX-XX\% Hits).

In summary, we present \model: a \underline{P}re-training warming up and \underline{E}nd-to-end training of subgraph \underline{R}etriever and \underline{R}easoner. The contributions of the work include:
\begin{itemize}
    \item A two-step retrieving plus reasoning framework for KBQA.
    \item An simple but efficient dual-encoder as the retriever.
    \item An EM-based end-to-end training method for optimizing both the retriever and the reasoner.
    \item An un- plus weak-supervised cascading pre-training strategy for warming up the retriever.

\end{itemize}




%The core of KBQA is to bridge the gap between the textural questions and the structured KBs. Ideally, a question is expected to be mapped into a subgraph of the KB. For example, the subgraph in Figure~\ref{fig:subgraph} is a query graph corresponding to the question ``Where did Canadian citizens with Turing Award graduate?''. Then the answers ``Edinburgh'', ``Cambriday'', and ``McGill'' can be easily obtained from the query graph. One popular kind of methods, called semantic parsing-based (SP-based) methods~\cite{lan-jiang-2020-query,sun2020sparqa}, focus on obtaining the exact subgraph that can be directly executed against the KBs. In contrast, the embedding-based methods relax the restriction of the exact subgraph by representing the questions and the entities on the whole KBs~\cite{chen2019bidirectional,miller2016key,qiu2020stepwise,saxena-etal-2020-improving,xu-etal-2019-enhancing,zhou-etal-2018-interpretable} or on the ad-hoc retrieved subgraphs~\cite{He_2021,sun-etal-2018-open} into the same embedding space and then reason the answer in the unified space by advanced deep learning methods such as GNN~\cite{sun-etal-2018-open} and neural state machine~\cite{chen2019bidirectional,He_2021}. 
%The SP-based methods are less fault-tolerant, as they rely heavily on the accuracy of the parsed executable subgraph. The embedding-based methods reinforce the role of the embedding-based reasoning but underestimate the quality of the subgraphs, which might affect the question answering accuracy and also lack the interpretability of the answers. None of the methods reinforce both the accuracy of the subgraphs and the powerful reasoning capability on the subgraphs. Some embedding-based method, such as PullNet~\cite{SunACL2019}, enhances the accuracy of the subgraphs by learning a subgraph retrieving model, but the answer reasoning module is reduced into classifying the nodes at the last retrieving step as the answer or not. 
